Lying Your Way to Better Traffic Engineering

To optimize the flow of traffic in IP networks, operators do traffic engineering (TE), i.e., tune routing-protocol parameters in response to traffic demands. TE in IP networks typically involves configuring static link weights and splitting traffic between the resulting shortest-paths via the Equal-Cost-MultiPath (ECMP) mechanism. Unfortunately, ECMP is a notoriously cumbersome and indirect means for optimizing traffic flow, often leading to poor network performance. Also, obtaining accurate knowledge of traffic demands as the input to TE is elusive, and traffic conditions can be highly variable, further complicating TE. We leverage recently proposed schemes for increasing ECMP's expressiveness via carefully disseminated bogus information ("lies") to design COYOTE, a readily deployable TE scheme for robust and efficient network utilization. COYOTE leverages new algorithmic ideas to configure (static) traffic splitting ratios that are optimized with respect to all (even adversarially chosen) traffic scenarios within the operator's "uncertainty bounds". Our experimental analyses show that COYOTE significantly outperforms today's prevalent TE schemes in a manner that is robust to traffic uncertainty and variation. We discuss experiments with a prototype implementation of COYOTE.

==> 250-model.tex <==
\section{Formal Model and Problem Formulation}\label{app:notation-problem}

We formally introduce our notation and define the \obliviousperdestination problem.

\vspace{.1in}
\noindent\textbf{Notation and terminology. } Let $G=(V,E)$ be a directed capacitated graph, where $c_e$ is the capacity of edge $e$.
%  Let $\vec G$ be the directed (non-capacited) representation of $G$, where each (unoriented) edge of $G$ is replaced by two directed edges with opposite directions. 
For each vertex $t \in V$ and each edge $e$, let $H_{t,e}$ be $1$ if $e$ is contained in the the per-destination DAG used to route traffic towards $t$, $0$ otherwise. 
%$H$ is given as as input. 
Let $E_t$ be the set of edges such that $a\in E_t$ if $H_{t,a}=1$.
For each vertex $t \in V $, for each edge $e=(u,v) \in E$, let $\phi_{t}(e)$ be the fraction the flow to $t$ entering vertex $u$ that is forwarded through $e$. Clearly, the \emph{splitting ratio} constraint, i.e., $\sum_{(v,u)\in E_t} \phi_t((v,u)) = 1$ and the \emph{acyclicity} constraint, i.e.,  at least one edge $a$ in each directed cycle of $G$ is such that $\phi(a)=0$, must hold. Let $f_{s,t}(v)$, for vertices $s,t,v \in V$, be the fraction of the demand $s \rightarrow t$ that enters $v$. Hence, $f_{s,t}(v)=\sum_{e=(u,v) \in E_t}  f_{s,t}(u) \phi_t(e)$ if $v \neq s$, $1$ otherwise.
% 
% \[ f_{s,t}(v) = \left\{
% \begin{array}{l l}
% \sum_{u|(u,v)\in H_t}  f_{s,t}(u) \phi_t((u,v)) & \text{if } v\neq s\\
% 1 & \text{otherwise}
% \end{array} \right.\]
%
When demand $d_{s,t}$ is routed from $s$ to $t$, its contribution to the flow on link $(u,v)$ is $d_{s,t}f_{s,t}(u)\phi_t((u,v))$. If $\phi$ and $f$ satisfy the above constraints, we say that $\phi$ is a {\em per-destination} (PD) routing through the given DAGs (as defined by $H$). We also say that $(\phi,f)$ is a PF routing, where $f$ clearly directly depends on the splitting ratios $\phi$. 

\vspace{.1in}
\noindent\textbf{Oblivious performance ratio~\cite{4032716}. } Given a Traffic Matrix (TM) $D=\{d_{s_1,t_1},\dots,d_{s_k,t_k}\}$ specifying the demand between each pair of vertices, the {\em maximum link utilization} induced by a PD routing $(\phi,f)$ is

\begin{displaymath}
MxLU(\phi,D)=\max_{e=(u,v)\in E}\nicefrac{\sum_{s,t\in D}d_{st}f_{s,t}(u)\phi_t(e)}{c_{e}}\text{.} 
\end{displaymath}

An {\em optimal} routing for $D$ is a PD routing that minimizes the load on the most utilized link, i.e.,

\begin{displaymath}
OPTU(D)=\min_{\phi |\phi \text{ is a PD routing}} MxLU(\phi,D)\text{.}
\end{displaymath}

The {\em performance ratio} of a given PD routing $\phi$ on a given TM $D$ is $PERF(\phi,\{D\})=\nicefrac{MxLU(\phi,D)}{OPTU(D)}$. Given a set ${\cal D}$ of TMs, the performance ratio of a PD routing $\phi$ on ${\cal D}$ is $PERF(\phi,{\cal D})=\max_{D\in {\cal D}}PERF(\phi,\{D\})$.
%  
% Observe that the performance ratio is always at least $1$. 
% The definition of performance ratio is based on the standard ``competitive analysis'', where the performance guarantees of a certain solution is given with respect to the best possible solution for the actual input of the problem. 
% As such, g
%   
%  
A routing $\phi$ is {\em optimal} if $PERF(\phi,{\cal D})\le PERF(\phi',{\cal D})$ for any $\phi'$.

The \obliviousperdestination problem is computing a PD routing $\phi$ that is optimal with respect to the given set ${\cal D}$ of TMs.
% Observe that the performance ratio is invariant to any proportional rescaling of the TMs or link capacities. 
The \obliviousperdestination can be formulated with the following non-linear minimization problem. 
%We first formulate below  \obliviousperdestination as a non-linear program for the oblivious performance scenario and then we describe the modifications needed to deal with bounded TMs. 
%\begin{align}
%& \min  \  \alpha \nonumber\\
%&  (\phi,f) \text{ is a PD routing} \nonumber\\
%& \forall \text{ edges } e=(u,v): \nonumber \\
%& ~~~~\forall \text{ TMs }D \text{ with } \lambda>0 \nonumber \\
%& ~~~~~~~~OPTU(D)=1 \text{ and } \forall i,j \lambda a_{i,j}\le d_{i,j}\le b_{i,j} : \nonumber  \\
%& ~~~~~~~~~~~~  \nicefrac{\sum_{(s,t)} d_{s,t}f_{s,t}(u)\phi_t(e)}{c(e)} \le \alpha  \nonumber
%\end{align}
\begin{align}
& \min  \  \alpha \nonumber\\
&  (\phi,f) \text{ is a PD routing} \nonumber\\
& \forall \text{ edges } e=(u,v): \nonumber \\
& ~~\forall \text{ TMs }D \in {\cal D} \text{ with } OPTU(D)=r: \nonumber  \\
& ~~~~  \nicefrac{\sum_{(s,t)} d_{s,t}f_{s,t}(u)\phi_t(e)}{c(e)} \le \alpha r  \nonumber
\end{align}

In this paper, as in~\cite{4032716}, we focus on those sets of demands that can be defined with linear constraints, which expressive enough to model traffic uncertainty, yet allowing us to simplify the complexity of the optimization problem. In particular, 
 the actual demand $d_{i,j}$ from a vertex $i$ to $j$ can assume any value in the range $a_{i,j} \le d_{i,j} \le b_{i,j}$, where $a_{i,j}$ and $b_{i,j}$ are the uncertainty bounds for $d_{i,j}$ and are given as an input to the problem.
  
 As in~\cite{4032716}, by observing that the performance ratio is invariant to any proportional rescaling of the TMs or link capacities, we can reformulate our problem as follows
%
\begin{align}
& \min  \  \alpha \nonumber\\
&  (\phi,f) \text{ is a PD routing} \nonumber\\
& \forall \text{ edges } e=(u,v): \nonumber \\
& ~~\forall \text{ TMs }D \in {\cal D} \text{ with } \lambda>0 \text{ such that:}\nonumber \\
& ~~~~OPTU(D)=1 \text{ and } \forall i,j\ \lambda a_{i,j}\le d_{i,j}\le \lambda b_{i,j} : \nonumber  \\
& ~~~~~~  \nicefrac{\sum_{(s,t)} d_{s,t}f_{s,t}(u)\phi_t(e)}{c(e)} \le \alpha  \nonumber
\end{align}

\noindent where $\lambda$ is used to scale each demand $D$ in ${\cal D}$ so that $OPTU(D)=1$.

When ${\cal D}$ is the set of all possible TMs, the performance ratio is referred to as the {\em oblivious} performance ratio. In that case, for each demand $d_{i,j}$, we can simply replace $a_{i,j}\le d_{i,j}\le \lambda b_{i,j}$ with $0 \le d_{i,j}$.
%In that case, we consider only TMs with $OPTU(D)=1$ since the performance ratio is invariant to any proportional rescaling of the TMs or link capacities. 

\eat{
		%
		\allowdisplaybreaks
		\begin{align}
		& \min  \  \alpha \nonumber\\
		&  (\phi,f) \text{ is a PD routing} \nonumber\\
		& \forall \text{ edges } e=(u,v)\text{, } \forall \text{ TMs }D \text{ with } OPTU(D)=1: \nonumber \\
		&  ~~~~ \nicefrac{\sum_{(s,t)} d_{s,t}f_{s,t}(u)\phi_t(e)}{c(e)} \le \alpha  \label{eq:constraints}
		\end{align}
		%\vspace{-1.3em}
		
		
		
		We consider only TMs with $OPTU(D)=1$ since the performance ratio is invariant to any proportional rescaling of the TMs or link capacities. 
		
		When restricting the set of admissible TMs to a set ${\cal D}$, where each demand $d_{i,j}$ from vertex $i$ to $j$ is bounded within $a_{i,j}\le d_{i,j}\le b_{i,j}$, the \obliviousperdestinationdag turns into the following formulation. The transformation is analogous to the one described in~\cite{4032716}. 
		%as in the \emph{margin model}, where a a margin of uncertainty of $x$, over a base traffic $d_{i,j}$ from vertex $i$ to $j$, means that the actual flow from $i$ to $j$ can be any value between $\frac{d_{i,j}}{x}$ and $x\cdot d_{i,j}$, the formulation of the problem becomes as follows.
		%
		\begin{align}
		& \min  \  \alpha \nonumber\\
		&  (\phi,f) \text{ is a PD routing} \nonumber\\
		& \forall \text{ edges } e=(u,v): \nonumber \\
		& ~~~~\forall \text{ TMs }D \text{ with } \lambda>0 \nonumber \\
		& ~~~~~~~~OPTU(D)=1 \text{ and } \forall i,j \lambda a_{i,j}\le d_{i,j}\le b_{i,j} : \nonumber  \\
		& ~~~~~~~~~~~~  \nicefrac{\sum_{(s,t)} d_{s,t}f_{s,t}(u)\phi_t(e)}{c(e)} \le \alpha  \nonumber
		\end{align}
		
		In the ``margin uncertainty'' model described in Sect.~\ref{sec:eval}, we used the above model where $d_{i,j}$ is the base traffic demand from vertex $i$ to $j$ and $a_{i,j}=\frac{d_{i,j}}{x}$ and $b_{i,j}=xd_{i,j}$
}


==> 270-formal-motivating-example.tex <==
\vspace{.1in}
\noindent
\textbf{Revising the motivating example. }%\label{sect:app-golden-ratio}
%
We show how the optimal per-destination (PD) routing for the example instance of Fig.~\ref{fig:COYOTE-overview} can be computed via a simple analysis of inequalities of the second order. 

It should first be observed that, in general, the set of demands that can be routed without exceeding the capacities of the edges of a network is always a polyhedral that can be described with linear constraints. In our case, this set if represented by $\{(d_{s_1,t},d_{s_2,t}) | d_{s_1,t} + d_{s_2,t} = 2\}$. As observe in Appendix~\ref{app:notation-problem}, we only consider two demands
$d_1=\{(d_{s_1,t},d_{s_2,t})=(2,0)\}$ and $d_2=\{(d_{s_1,t},d_{s_2,t})=(0,2)\}$, which are the vertices of the demands polyhedral.
We denote by $load(e)$ the worse-case link utilization on an edge $e$ and by $\phi((u,v))$ the fraction of the flow to $t$ entering vertex $u$ that is forwarded towards $v$.
We observe that $load(s_1,v)\le load(v,t)$ and $load(s_2,v)\le load(v,t)$ since link $(v,t)$ carries the incoming flows from $(s_1,v)$ and $(s_2,v)$.

We now compute the amount of flow routed through the remaining links for the two demands. As for $d_1$, the most congested edge must be either $(s_1,s_2)$ or $(v,t)$ since $(s_2,t)$ carries no more traffic than $(s_1,s_2)$. We have that

\begin{align}
load(s_1,s_2) &\ge 2 \phi(s_1,s_2) \label{eq:s1-s2} \\
load(v,t) & \ge 2(1 - \phi(s_1,s_2)) + 2\phi(s_1,s_2) (1-\phi(s_2,t)) \nonumber \\
& \ge 2(1 - \phi(s_1,s_2) \phi(s_2,t)) \label{eq:v-t}
\end{align}

As for demand $d_2$, we observe that the most congested edge is either $(s_2,t)$ or $(v,t)$, where:

\begin{align}
load(s_2,t) & \ge 2 \phi(s_2,t)  \label{eq:s2-t} \\
load(v,t) & \ge 2(1 - \phi(s_2,t)) \label{eq:v-t-2}
\end{align}

As for $load(v,t)$, we observe that $ 2(1 - \phi(s_1,s_2) \phi(s_2,t)) \ge  2(1 - \phi(s_2,t))$, for any $0\le \phi(s_2,t) \le 1$, which
means that~\ref{eq:v-t-2} is obsolete.

We want to balance the congestion among  links $(s_1,s_2)$, $(s_2,t)$, and $(v,t)$ for . Observe that (\ref{eq:s1-s2}) increases w.r.t. $\phi(s_1,s_2)$,(\ref{eq:s2-t}) increases w.r.t. $\phi(s_2,t)$, while (\ref{eq:v-t}) decreases w.r.t. both $\phi(s_1,s_2)$ and $\phi(s_2,t)$. As such, to minimize the most utilized link, inequalities (\ref{eq:s1-s2}), (\ref{eq:s2-t}),and (\ref{eq:v-t}) must be tight in the optimal case, i.e., $load(s_1,s_2)=load(s_2,t)=load(v,t)$
%
%\begin{align}
%load(s_1,s_2) & = 2 \phi(s_1,s_2) \nonumber \\
%load(v,t) & = 2(1 - \phi(s_1,s_2) \phi(s_2,t)) \nonumber \\
%load(v,t) & \ge 2\phi(s_2,t) \nonumber
%\end{align}
%
Moreover, inequalities (\ref{eq:s1-s2}) and (\ref{eq:s2-t}) imply that $\phi(s_1,s_2)= \phi(s_2,t)$, which allows us to rewrite (\ref{eq:v-t}) as $load(v,t)=1 - \phi(s_1,s_2)^2$. From (\ref{eq:s1-s2}) and~\ref{eq:v-t}, we have that $  2\phi(s_1,s_2) = 2(1 - \phi(s_1,s_2)^2) \rightarrow
  1 - \phi(s_1,s_2) -\phi(s_1,s_2)^2 =0 $, which is an equation of the second order with solutions $\frac{\sqrt{5}-1}{2}$ and $\frac{\sqrt{5}+1}{2}$,
%
%$$\phi_1(s_1,s_2)=\frac{\sqrt{5}-1}{2} \sim 1,618 \mbox{; } \phi_2(s_1,s_2)=\frac{\sqrt{5}+1}{2} \sim 0,618$$
%
%\noindent
 where only the second solution (i.e., the inverse of the golden ratio) is feasible in our formulation. The optimal splitting ratios are therefore $ \phi(s_1,s_2)= \frac{\sqrt{5}-1}{2} \mbox{ and } \phi(s_2,t)= -\frac{\sqrt{5}+1}{2}$, where the most congested edge for any permitted traffic matrix is at most $\sqrt{5}-1\sim 1,23$. COYOTE correctly finds this solution.


==> signomial.tex <==
\subsection{Given a DAG - Oblivious Routing}
    
In this subsection, we study the oblivious per-destination problem, in which a set of per-destination directed acyclic subgraphs (DAG) of $\vec G$ is given, where $\vec G$ is the oriented copy of $G$ in which each unoriented edge $e$ is replaced by two opposite arcs each with capacity $c(e)$. Routing towards a destination vertex must be computed according to the orientation of the edges of a specific DAG.

\newpage
\subsubsection{Per-destination oblivious routing (Ami)}

Let $G$ be a capacited directed graph, where $c(e)$ is the capacity of arc $e$, $D$ be a set of pairs of source-destinations vertices, and $k\ge1$ be a constant. For each destination vertex $t \in V(G)$, let  $H_t$ be a directed acyclic subgraph (DAG) of $G$. Routing towards a destination vertex must be computed according to the orientation of the edges of a specific DAG.

Let $f_{s,t}(v)$ be the fraction of the flow from $s$ to $t$ that arrives at vertex $v$, and, for each outgoing arc $(v,u)$ in $H_t$, let $\phi_t((v,u))$ be the fraction of $f_{s,t}(v)$ that is sent through $(v,u)$. A {\em per-destination routing} is uniquely defined by the splitting ratios variables. 

\vspace{.1in}
\noindent\textbf{Flow constraints.}
The fraction of the flow from $s$ to $t$ that arrives at vertex $v$ can be computed as follows:

%$$f_{s,t}((u,v)) \ge \phi_t((u,v)) F_{IN}, $$
\[ f_{s,t}(v) = \left\{
  \begin{array}{l l}
    \sum_{u|(u,v)\in H_t}  f_{s,t}(u) \phi_t((u,v)) & \text{if } v\neq s\\
    1 & \text{otherwise}
  \end{array} \right.\]
  
\noindent , where we sum up all the flow contributions from each incoming arc at $v$, if $v\neq s$. If $v=s$, then $v$ must spread the entire $(s,d)$-flow among its outgoing edges.

The second flow constraints is used to guarantee that the sum of the splitting ratios at a certain vertex $v$ towards a destination $t$ is $1$:
$$\sum_{(v,u)\in E(H_t)} \phi_t((v,u)) = 1 .$$
  
 \vspace{.1in}
 \noindent\textbf{The admissible set of demand matrices. } So far, we only considered fractions of flows between any source-destination pair without specifying the exact amount that must be routed between the two endpoints. We now define the set of demand matrices $\cal{D}$ that we want to handle with our per-destination oblivious routing. A demand matrix $\{d_{s,t}|d_{s,t} \in \mathbb{R}^+_{\geq 0}, \forall (s,t) \in D \}$ is in $\cal{D}$, where $d_{s,t}$ is the amount of flow that must be routed from $s$ to $t$, if, intuitively, all the flows can be routed without exceeding the capacities of the edges. Namely, the following constraints must be satisfied:
 
 \[ \left\{
 \begin{array}{l l}
   \sum_{a\in IN(v)} g_t(a) - \sum_{a\in OUT(v)} g_t(a) +d_{v,t} = 0 & \forall t \in T, \forall v\neq t \in V(G)\\
\sum_{t\in T} g_t(a) \le c(a)  & \forall a \in E( G)
  \end{array} \right. \]
 
 \noindent, where $g_t(a)$ represents the amount of flow (not the fraction) directed to $t$ that is routed through arc $a$. The first constraint is a flow conservation constraint, while the second one is an arc capacity constraint. We denote by $D_1,\dots,D_k$ the set of vertices of the polyhedral $\cal{D}$ and we consider only these demands. Each $D_i$ defines the amount of flow to be routed between each pair in $D$. We denote by $d_{s,t,i}$  the amount of flow from $s$ to $t$ in $D_i$.
 
 We have that the amount of flow that is routed through an edge $(u,v)$ for a demand $D_i$ is:
 
 $$\sum_{(s,t)\in D} d_{s,t,i}f_{s,t}(u)\phi_t((u,v)),$$
 
\noindent and the {\em} load on the edge is:
 
 $$l((u,v)) = \frac{\sum_{(s,t)\in D} d_{s,t}f_{s,t,i}(u)\phi_t((u,v))}{c(e)}.$$
 
 
  \vspace{.1in}
  \noindent\textbf{Formulation with an exponential number of constraints.}
  

 \begin{align}
\min & \  cost(l(e_1),\dots,l(e_{|E( G)|}))&\\
&     f_{s,t}(v) \ge \left\{
  \begin{array}{l l}
    \sum_{u|(u,v)\in H_t} f_{s,t}(u) \phi_t((u,v))  & \text{if } v\neq s\\
    1 & \text{otherwise}
  \end{array} \right. && \forall (s,t) \in D, \forall v\neq t \in V(H_t)\\
&  \sum_{(v,u)\in E(H_t)} \phi_t((v,u)) \ge 1 && \forall t \in T, \forall v \in V(H_t)\\
&   l((u,v)) \ge \frac{\sum_{(s,t)\in D} d_{s,t,i}f_{s,t}(u)\phi_t((u,v))}{c(e)}  && \forall{D_i \in \cal{D}}, \forall (u,v) \in E(G)\\
%&\left\{\begin{aligned}
%  w^{ij} c \le \alpha &&&\forall (s,t) \in S \\
%  \pi^{ij}_{st,v} - \pi^{ij}_{st,u} \le w^{ij}_{uv} &&&\forall (s,t) \in S, \forall (u,v) \in E\\
% \pi^{ij}_{st}(e_t - e_s) \ge \frac1{c_{ij}}\sum_{k=1}^Kx^k_{st,ij} &&& \forall (s,t) \in S\\
%  w^{ij} \ge 0
%\end{aligned}\right\} && \forall (i,j) \in E\\
&   \text{\% all variables are greater than or equal to 0.}
  \end{align}
  
  The $cost$ function has in input the load of each arc and it outputs a measure of the congestion of the network. We consider two different cost functions:
  
  \begin{itemize}
  \item {\em The most loaded arc}. Namely, $max_{e\in E} l(e)$. 
  \item {\em The sum of link costs}. Namely, $sum_{e\in E} edge\_cost(l(e))$, where $edge\_cost$ must be a convex function of the load on an arc. We need a convex function because we want to spread the flow of traffic as evenly as possible, avoiding very loaded arcs. 
  \end{itemize}
  
  
  
 \vspace{.1in}
 \noindent\textbf{Our approach so far: separation oracle and signomial programming.}
For the first objective function  (i.e., most loaded arc)  we know how to compute a solution (not necessarily optimal) using a signomial programming approach + dual of a separation oracle but it does not scale because of the size of the separation oracle (see below). For the second objective (i.e., sum of link costs), we cannot design a linear programming separation oracle. If we could, then we could probably compute good solutions for large networks as well.
 
 Let's  first consider the most loaded arc optimization function. Using a standard approach, we can remove the exponential many constraints and replace them with the dual of a separation oracle, which we now describe. Given a feasible solution, the separation oracle outputs a demand matrix that creates the highest load/congestion on an arc. Namely, for each arc $e \in E(G)$, we  solve the following linear programming ($f$ and $\phi$ are constants here) in order to find a set of demands that is routable with load at most 1 and that maximize the load on arc $e=(u,v)$:
 
 \begin{align}
\max &  \   \frac{\sum_{(s,t)\in D} d_{s,t,i}f_{s,t}(u)\phi_t((u,v))}{c(e)} &\\
&    \sum_{a\in IN(v)} g_t(a) - \sum_{a\in OUT(v)} g_t(a) +d_{v,t} \le 0 && \forall t \in T, \forall v\neq t \in V(G)\\
& \sum_{t\in T} g_t(a) \le c(a)  && \forall a \in E(G)\\
%&\left\{\begin{aligned}
%  w^{ij} c \le \alpha &&&\forall (s,t) \in S \\
%  \pi^{ij}_{st,v} - \pi^{ij}_{st,u} \le w^{ij}_{uv} &&&\forall (s,t) \in S, \forall (u,v) \in E\\
% \pi^{ij}_{st}(e_t - e_s) \ge \frac1{c_{ij}}\sum_{k=1}^Kx^k_{st,ij} &&& \forall (s,t) \in S\\
%  w^{ij} \ge 0
%\end{aligned}\right\} && \forall (i,j) \in E\\
&   \text{\% all variables are at least 0.}
  \end{align}
  
  Constraints (7) and (8) are used to guarantee that the demands can be routed with load at most 1.
  
  The dual for a specific arc $e\in E$ is (where we create a dual variable $\pi_{v,t}(e)$ to each constraint of type (7) and a dual variable $w_e(a)$ to each constraint of type (8):
  
   \begin{align}
  \min &\  \sum_{a\in \{a|\cup_{t\in T} E(H_t)\}} w_e(a)c(a)  && \\
&     w_e((v,u))  + \pi_{u,t}(e) - \pi_{v,t}(e) \ge 0 &&  \forall t \in T, \forall (v,u) \in E(H_t)\\
&     w_e((v,u)) - \pi_{v,t}(e)  \ge 0  &&  \forall (v,t) \in E(H_t)\\
&    c(e)\pi_{s,t}(e)  \ge  f_{s,t}(u)\phi_{t}((u,v)) &&  \forall t \in T, \forall (s,t) \in D\\
&   \text{\% all variables are at least 0.}
\end{align}
 
  Observe that, for each edge $e\in E$, we can now plug its dual in the original formulation, which leads to the following formulation:
  
 \begin{align}
&    \min \max_{e\in E} \sum_{a\in \{a|\cup_{t\in T} E(H_t)\}} w_e(a)c(a)&\\
&     f_{s,t}(v) \ge \left\{
  \begin{array}{l l}
    \sum_{(u,v)\in E(H_t)} f_{s,t}(u)\phi_t((u,v))  & \text{if } v\neq s\\
    0 & \text{otherwise}
  \end{array} \right. && \forall (s,t) \in D, \forall v\neq t \in V(H_t)\\
&  \sum_{(v,u)\in E(H_t)} \phi_t((v,u)) \ge 1 && \forall t \in T, \forall v \in V(H_t)\\
&     w_{e}((v,u))  + \pi_{u,t}(e) - \pi_{v,t}(e) \ge 0 && \forall e \in E(\vec G), \forall t \in T, \forall (v,u) \in E(H_t)\\
&     w_{e}((v,u)) - \pi_{v,t}(e)  \ge 0  && \forall e \in E(\vec G), \forall (v,t) \in E(H_t)\\
&    c(e)\pi_{s,t}(e)  \ge  f_{s,t}(u)  \phi_{t}((u,v)) && \forall e=(u,v) \in E(\vec G), \forall t \in T, \forall (s,t) \in D\\
%&\left\{\begin{aligned}
%  w^{ij} c \le \alpha &&&\forall (s,t) \in S \\
%  \pi^{ij}_{st,v} - \pi^{ij}_{st,u} \le w^{ij}_{uv} &&&\forall (s,t) \in S, \forall (u,v) \in E\\
% \pi^{ij}_{st}(e_t - e_s) \ge \frac1{c_{ij}}\sum_{k=1}^Kx^k_{st,ij} &&& \forall (s,t) \in S\\
%  w^{ij} \ge 0
%\end{aligned}\right\} && \forall (i,j) \in E\\
&   \text{\% all variables are at least 0.}
  \end{align}

\
  
  The resulting formulation has a polynomial number of constraints. We use a signomial programming approximation technique to deal with the quadratic constraints contained in Constraint (\ref{}). 
  The main issue is that this formulation has $O(|E|^2|V|)$ many constraints, which makes it hard to solve for networks with hundreds of edges. 
  
  To solve the scalability problem, we tried to reduce the number of constraints that comes from the dual problems associated with the separation oracle by changing the optimization function. If we could find a separation oracle for the second objective function, then we could obtain a much smaller formulation since we do not have to try to maximize the load on each single arc independently. This would scale to large networks. However, the following maximization problem, which would be a separation oracle for the second objective function, is not convex (this is the problem that I asked you the very first day we met):
 
 
  
   \begin{align}
\max &  \sum_{e\in E} edge\_cost\left(\frac{\sum_{(s,t)\in D} d_{s,t}f_{s,t}(u)\phi_t((u,v))}{c(e)}\right) &\\
&    \sum_{a\in IN(v)} g_t(a) - \sum_{a\in OUT(v)} g_t(a) +d_{v,t} \le 0 && \forall t \in T, \forall v\neq t \in V(G)\\
& \sum_{t\in T} g_t(a) \le c(a)  && \forall a \in E( G)\\
%&\left\{\begin{aligned}
%  w^{ij} c \le \alpha &&&\forall (s,t) \in S \\
%  \pi^{ij}_{st,v} - \pi^{ij}_{st,u} \le w^{ij}_{uv} &&&\forall (s,t) \in S, \forall (u,v) \in E\\
% \pi^{ij}_{st}(e_t - e_s) \ge \frac1{c_{ij}}\sum_{k=1}^Kx^k_{st,ij} &&& \forall (s,t) \in S\\
%  w^{ij} \ge 0
%\end{aligned}\right\} && \forall (i,j) \in E\\
&   \text{\% all variables are at least 0.}
  \end{align}
  
  Let's compute the Wolff dual of this non-convex problem, where $edge\_cost(x) = x^2$:
  
   \begin{align}
\min &   \sum_{(u,v)\in E} \left(\frac{\sum_{(s,t)\in D} d_{s,t}f_{s,t}(u)\phi_t((u,v))}{c(e)}\right)^2 - \\
& - \sum_{(s,t)\in S} \pi_{s,t} d_{s,t}  - \sum_{a\in E(G)} w_ac(a)&& \\
& \sum_{e\in E} \left( 2 \frac{\sum_{(s,t)\in D} d_{s,t}f_{s,t}(u)\phi_t((u,v))}{c(e)}\left(\frac{f_{s,t}(u)\phi_t((u,v))}{c(e)} \right) \right) = \pi_{s,t} && \forall (s,t) \in S \\
&     w_e((v,u))  + \pi_{u,t}(e) - \pi_{v,t}(e) = 0 &&  \forall t \in T, \forall (v,u) \in E(H_t)\\
&     w_e((v,u)) - \pi_{v,t}(e)  = 0  &&  \forall (v,t) \in E(H_t)\\
&   \text{\% all variables are at least 0.}
\end{align}
  
 \newpage
\subsubsection{General formulation}
\noindent\textbf{Variables: }
\begin{itemize}
 \item $f_{s,t}(v)$, for each pair $(s,t) \in D$ and each vertex $v\neq t \in V(H_t(s))$. It represents the fraction of the flow from $s$ to $t$ that is entering at $v$.
 \item $\phi_{t}(e)$, for each destination $t \in T $, for each arc $e\in E(H_t)$. It represents the fraction of the incoming flow at vertex $u$, where $e=(u,v)$, that is sent through $e$.
\end{itemize}

\subsubsection{Signomial Approach}

\vspace{.1in}
\noindent\obliviousperdestinationdag
\begin{itemize}
\item  \textbf{Instance}: A capacited graph $G$, where $c(e)$ is the capacity of edge $e$, a set $D$ of pairs of source destinations,  for each destination vertex $t \in V(G)$, a directed acyclic subgraph $H_t$ of $\vec G$, and a constant $k\ge1$.
\item \textbf{Problem}: Does there exist a per-destination routing such that the oblivious performance is at most $k$?
\end{itemize}

 We now design a signomial programming formulation of the problem and design an iterative geometric algorithm based on approximating the signomial constraints with posynomials constraints.

 We compare the oblivious per-destination performance against the oblivious source-destination oblivious performance on the same DAG. Otherwise, the gap is know to be arbitrarily large.
 
 We assume that each vertex in $H_t$ does not have any incoming arcs if and only if it is a source vertex towards $t$.
 
\vspace{.1in}
\noindent\textbf{Additional notatation:}
 \begin{itemize}
 %\item Let $H_t(e)$ be the subgraph of $H_t$ such that it contains all and only the paths through $e$ that end at $t$. Namely, an arc $a$ is in $E(H_t(e))$ iff there exists a path to $t$ that traverses both $a$ and $e$ (in any order). Analogously, a vertex is in $V(H_t(e))$ iff there exists a path to $t$ that traverses both $e$ and $v$ (in any order).
 \item Let $H_t(s)$ be the subgraph of $H_t$ such that  it contains all and only the paths from the source vertex $s$ to the destination $t$. Namely, an arc $(u,v)$ is in $E(H_t(s))$  iff there exists a path from $s$ to $t$ through $(u,v)$.
 \item Let $S_t(e)$ be the set of source vertices $s$ sucht that $(s,t) \in D$ and there exists a path from $s$ to $t$ through $e$.
 \item Let $T$ be the set of destination vertices.
 %\item Let $IN(v)$ ($OUT(v)$) be the set of incoming (outgoing) arcs at vertex $v$.
\end{itemize}

\vspace{.1in}
\noindent\textbf{Variables: }
\begin{itemize}
% \item $d_{s,t}$, for each pair $(s,t) \in {\cal D} $. It represents the amount of flow that must be routed from vertex $s$ to vertex $t$.
 \item $f_{s,t}(v)$, for each pair $(s,t) \in D$ and each vertex $v\neq t \in V(H_t(s))$. It represents the fraction of the flow from $s$ to $t$ that is entering at $v$.
 \item $\phi_{t}(e)$, for each destination $t \in T $, for each arc $e\in E(H_t)$. It represents the fraction of the incoming flow at vertex $u$, where $e=(u,v)$, that is sent through $e$.
 \item $\pi_{v,t}(e)$, for each  $t \in T$, for each $v\neq t \in V(H_t)$. It is a dual variable of the separation oracle. It represents the potential at node $v$ from the target $t$ where the goal is to maximize congestion on edge $e$. 
 \item $w_{e}(a)$, for each $e \in E(\vec G)$, for each $a\in \{a|\cup_{t\in T} E(H_t)\}$. It is a dual variable of the separation oracle. It represents the weight of arc $a$ where the goal is to maximize congestion on edge $e$. 
 \item $\alpha$. It represents the most congested edge.
\end{itemize}

\vspace{.1in}
\noindent\textbf{Objective: }

$$\min \alpha$$

\vspace{.1in}
\noindent\textbf{Constraints: }

\begin{enumerate}
 \item\label{slight-change-constraint} For each demand $(s,t) \in D$, for each vertex $v \neq t \in V(H_t(s))$, the outgoing flow from  $v$ is spread among the outgoing edges based on the splitting ratio variables: 
%$$f_{s,t}((u,v)) \ge \phi_t((u,v)) F_{IN}, $$
\[ f_{s,t}(v) \ge \left\{
  \begin{array}{l l}
    \sum_{u|(u,v)\in E(H_t(s))} \phi_t((u,v)) f_{s,t}(u) & \text{if } v\neq s\\
    1 & \text{otherwise}
  \end{array} \right.\]
%$$F^{IN}_{s,t}(v) \ge \sum_{u|(u,v)\in E(H_t(s))} \phi_t((u,v)) F^{IN}_{s,t}(u), $$
%\noindent where $F_{IN}=1$ if $v=s$, $\sum_{(z,u)\in E(H_t(s))} f_{s,t}((z,u))$, otherwise.
 \item\label{non-gp-constraint} For each $t \in T$, for each $v \in V(H_t)$. The sum of the splitting ratios at a certain vertex $v$ towards a destination $t$ must be at least 1. Observe that we will rewrite this constraint in a different form as it is not in GP form:
$$\sum_{(v,u)\in E(H_t)} \phi_t((v,u)) \ge 1 .$$
 \item For each $e \in E(\vec G)$, this is the objective function of the dual of the separation oracle problem:
$$\alpha \ge \sum_{a\in \{a|\cup_{t\in T} E(H_t)\}} w_e(a)c(a) . $$
 \item For each $e \in E(\vec G)$, for each $t \in T$, for each $(v,u) \in E(H_t)$, this is the potential constraint:
$$\pi_{u,t}(e) - \pi_{v,t}(e) + w_{e}((v,u)) \ge 0.$$
 \item For each $e \in E(\vec G)$, for each $(v,t) \in E(H_t)$, this is the potential constraint for the edge case in which the head of the arc is the destination vertex:
$$ - \pi_{v,t}(e) + w_{e}((v,t)) \ge 0 .$$
 \item For each $e=(u,v) \in E(\vec G)$, for each $t \in T$, for each $(s,t) \in S_t(e)$, this is the potential requirement between the source and target vertex:
$$\pi_{s,t}(e)  \ge \frac{f_{s,t}(u)\phi_{t}((u,v))}{c(e)} .$$
\end{enumerate}

 An optimization problem is called a Mixed Linear Geometric Programming (MLGP) if with a log change of $x$ variables, the following problem can be turned into a convex optimization:

\begin{align*}
 \texttt{minimize }    & f_0(x) + a^T_0 y \\
 \texttt{subject to }  & f_i(x)+ a^T_i y + d_i \le 1 ,i =1 ,\dots,m\\
 \texttt{ } & h_j(x)=1 ,j =1 ,\dots,M \\ 
 \texttt{variables }   & x, y.
\end{align*}

\noindent where $f_i(x)$ is a sum of posynomials, $h_j(x)$ is a monomial, and both $a$ and $d$ are vectors of real numbers. We now show how to rewrite the previous constraints in a MLGP form.

We classify the variables and constraints defined in the previous formulation as follows. Variables that belong to the geometric programming, i.e., $x$ variables, are $f_{s,t}^e$ and $\phi_t(e)$, while variables that belong to the linear programming, i.e., $y$ variables, are $\alpha$, $\pi_{v,t}(e)$, and $w_e(a)$. 
Observe that constraint~\ref{slight-change-constraint} is the only pure GP constraint (we divide by $f_{s,t}(u,v)$ both sides). Constraints $3$-$5$ are linear programming constraints, while constraint $6$ is a MLGP constraint.
Only  constraint~\ref{non-gp-constraint} cannot be classified neither as a GP constraint nor a linear constraint. For this reason, we apply a standard technique in Signomial programming, called \emph{complementary GP}, to find a solution to the problem. This technique consists in iteratively performing two steps: (i) given a feasible solution, approximate every signomial constraint with a monomial, which makes the entire formulation a MLGP, and (ii) find a new optimal feasible point by solving the MLPG. Initially, a feasible point solution must be given in input. In our case, a random routing is sufficient. 

\vspace{.1in}
\noindent\textbf{Monomial Approximation of Constraint 2.}
%We are given a nonlinear function $f : R_n \rightarrow R$ that is differentiable at $x_0 \succ 0$ and $f(x_0) > 0$. We would like to approximate $f(x)$ with a monomial $\hat f(x)= c\prod^n_{i =1}x^{a_i}_i$. We use the following log transformation: $y_i = \log x_i$, $g(y) = \log f(y)$, $\hat g(y) = \log \hat f(y) = \log c + a^Ty$. Equating the first order Taylor expansion of $g$ at $y_0$ with $\hat g(y)$, we obtain:
Let $f_{v,t}(\phi)= \sum_{(v,u)\in E(H_t)} \phi_t((v,u))$, where $\phi$ is an array containing all the $\phi$ variables in the sum. We denote by $\phi(i)$ the $i$'th variable in $\phi$. Given a point $\phi_0$, we want to approximate $f_{v,t}$ with a monomial $\hat f_{v,t}(\phi)= k\prod^n_{i =1}(\phi(i))^{a(i)}$. Let $y = \log\phi$. From  the calculations in~\cite{} we have

$$a(i)=\left.\frac{\phi(i)}{f_{v,t}(\phi)}\frac{\partial f_{v,t}}{\partial \phi(i)}\right|_{\phi=\phi_0} = \frac{\phi_0(i)}{\sum_{i} \phi_0(i)}$$

\noindent and

$$k=\left.\frac{f_{v,t}(\phi)}{\prod_{i=1}^{n}{(\phi(i))^{a_i}}}\right|_{\phi=\phi_0} = \frac{\sum_{i} \phi_0(i)}{\prod_{i=1}^{n}{(\phi_0(i))^{a(i)}}}.$$

Hence, given a point $\phi_0$, constaint 2 is rewritten as:

$$ \frac{1}{k\prod^n_{i =1}(\phi(i))^{a(i)}}\le 1,$$

\noindent which is in GP form, since it is a monomial.

\subsubsection{Max-Congested-Edge: Convex formulation}

Given a feasible solution $<\hat \alpha,\hat \pi, \hat w,\hat \phi, \hat f>$, we can compute $a_t(u,v)$ and $k_t$, which leads to the following  formulation:

 \begin{align}
&    \min \alpha&\\
&     \tilde f_{s,t}(v) \ge \left\{
  \begin{array}{l l}
    \log \sum_{(u,v)\in E(H_t(s))} e^{\tilde \phi_t((u,v)) + \tilde f_{s,t}(u)} & \text{if } v\neq s\\
    0 & \text{otherwise}
  \end{array} \right. && \forall (s,t) \in D, \forall v\neq t \in V(H_t(s))\\
&     \log k_t +  \sum^n_{(v,u)\in E(H_t)}a_t(v,u)\tilde\phi_t((v,u))\ge 0  && \forall t \in T, \forall v \in V(H_t)\\
&    \alpha \ge \sum_{a\in \{a|\cup_{t\in T} E(H_t)\}} w_e(a)c(a)  && \forall e \in E(\vec G)\\
&     w_{e}((v,u))  + \pi_{u,t}(e) - \pi_{v,t}(e) \ge 0 && \forall e \in E(\vec G), \forall t \in T, \forall (v,u) \in E(H_t)\\
&     w_{e}((v,u)) - \pi_{v,t}(e)  \ge 0  && \forall e \in E(\vec G), \forall (v,t) \in E(H_t)\\
&    c(e)\pi_{s,t}(e)  \ge  e^{\tilde f_{s,t}(u) + \tilde \phi_{t}((u,v))} && \forall e=(u,v) \in E(\vec G), \forall t \in T, \forall (s,t) \in S_t(e)\\
%&\left\{\begin{aligned}
%  w^{ij} c \le \alpha &&&\forall (s,t) \in S \\
%  \pi^{ij}_{st,v} - \pi^{ij}_{st,u} \le w^{ij}_{uv} &&&\forall (s,t) \in S, \forall (u,v) \in E\\
% \pi^{ij}_{st}(e_t - e_s) \ge \frac1{c_{ij}}\sum_{k=1}^Kx^k_{st,ij} &&& \forall (s,t) \in S\\
%  w^{ij} \ge 0
%\end{aligned}\right\} && \forall (i,j) \in E\\
&   \text{\% variable constraints omitted}
  \end{align}

\eat{\subsubsection{Mosek formulation}

We use \texttt{MOSEK} to solve our MPLG formulation, in which each the argument of each non-linear function must contain a single variable . Given a feasible solution $<\hat \alpha,\hat \pi, \hat w,\hat \phi, \hat f>$, the final formulation is as follows:

 \begin{align}
&    \min \alpha&\\
&     \tilde f_{s,t}(v) \ge \left\{
  \begin{array}{l l}
    \log y_{s,t}(v) & \text{if } v\neq s\\
    0 & \text{otherwise}
  \end{array} \right. && \forall (s,t) \in D, \forall v\neq t \in V(H_t(s))\\
&  y_{s,t}(v) \ge \sum_{(u,v)\in E(H_t(s))} e^{g_{s,t}(u,v)} && \forall (s,t) \in D, \forall v\neq t \in V(H_t(s))\\
&  g_{s,t}(u,v) \ge \tilde \phi_t((u,v)) + \tilde f_{s,t}(u) && \forall (s,t) \in D, \forall  (u,v\neq t)\in E(H_t(s))\\
&      \sum^n_{(v,u)\in E(H_t)}a_t(v,u)\tilde\phi_t((v,u))\ge -\log k_t   && \forall t \in T, \forall v\neq t \in V(H_t)\\
&    \alpha \ge \sum_{a\in \{a|\cup_{t\in T} E(H_t)\}} w_e(a)c(a)  && \forall e \in E(\vec G)\\
&     w_{e}((v,u))  + \pi_{u,t}(e) - \pi_{v,t}(e) \ge 0 && \forall e \in E(\vec G), \forall t \in T, \forall (v,u\neq t) \in E(H_t)\\
&     w_{e}((v,u)) - \pi_{v,t}(e)  \ge 0  && \forall e \in E(\vec G), \forall (v,t) \in E(H_t)\\
&    c(e)\pi_{s,t}(e)  \ge \tilde f_{s,t}(u) + \tilde \phi_{t}((u,v)) && \forall e=(u,v) \in E(\vec G), \forall t \in T, \forall (s,t) \in S_t(e)\\
%&\left\{\begin{aligned}
%  w^{ij} c \le \alpha &&&\forall (s,t) \in S \\
%  \pi^{ij}_{st,v} - \pi^{ij}_{st,u} \le w^{ij}_{uv} &&&\forall (s,t) \in S, \forall (u,v) \in E\\
% \pi^{ij}_{st}(e_t - e_s) \ge \frac1{c_{ij}}\sum_{k=1}^Kx^k_{st,ij} &&& \forall (s,t) \in S\\
%  w^{ij} \ge 0
%\end{aligned}\right\} && \forall (i,j) \in E\\
&   \text{\% variable constraints omitted}
  \end{align}
}

  
  
  
  
  
  
  
  
  
  
  
  
  
